On completeness and parametricity in the realizability semantics of System F

We investigate completeness and parametricity for a general class of realizability semantics for System F defined in terms of closure operators over sets of $\lambda$-terms. This class includes most semantics used for normalization theorems, as those arising from Tait's saturated sets and Girard's reducibility candidates. We establish a completeness result for positive types which subsumes those existing in the literature, and we show that closed realizers satisfy parametricity conditions expressed either as invariance with respect to logical relations or as dinaturality. Our results imply that, for positive types, typability, realizability and parametricity are equivalent properties of closed normal $\lambda$-terms.

==> macros.tex <==
\newtheorem{theorem}{Theorem}[section]

\newtheorem{example}[theorem]{Example}
\newtheorem{convention}[theorem]{Convention}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{notation}[theorem]{Notation}

\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{falselemma}{False lemma}[section]

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{result}[theorem]{Result}

\numberwithin{equation}{section}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


\makeatletter
\newenvironment{proofof}[1]{
\par \pushQED{\qed} 
\normalfont \topsep6\p@\@plus6\p@\relax
\trivlist
\item[\hskip\labelsep \itshape
Proof of #1 \@addpunct{.}]\ignorespaces}{ %
\popQED\endtrivlist\@endpefalse}
\makeatother


\newtheorem{corollary}[theorem]{Corollary}

%math styles
\newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\TT}[1]{\mathtt{#1}}
\newcommand{\D}[1]{\mathscr{#1}}
\newcommand{\SF}[1]{\mathsf{#1}}

\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\BB}[1]{\mathbb{#1}}
\newcommand{\U}[1]{\underline{#1}}
\newcommand{\OV}[1]{\overline{#1}}
\newcommand{\F}[1]{\mathfrak{#1}}
\newcommand{\tr}{\trianglelefteq}
\newcommand{\To}{\Rightarrow}
\newcommand{\flow}{\ensuremath{\leftharpoonup}}		% flot symetrique: u<-v + v<-u
\newcommand{\vv}{\TT{var}}
\newcommand{\s}{\TT{subt}}
\newcommand{\hv}{\TT{hvar}}
\newcommand{\mm}[1]{{\color{red}#1}}

\newcommand{\arrow}[2]{\left (#1\To#2\right )}
\newcommand{\etanf}[2]{\lceil #1 \rceil_{#2}}
\newcommand{\sk}[0]{\mathsf{sk}}
\newcommand{\forpiudue}[0]{\forall^{+}}
\newcommand{\formenodue}[0]{\forall^{-}}
\newcommand{\forpiupro}[0]{\forall^{+}_{\TT P}}
\newcommand{\formenopro}[0]{\forall^{-}_{\TT P}}
\newcommand{\Cl}[0]{\mathfrak C}
\newcommand{\CR}[0]{\mathsf{CR}}
\newcommand{\CRuno}[0]{\mathsf{CR}'}
\newcommand{\CRdue}[0]{\mathsf{CR}''}
\newcommand{\Rel}[2]{\langle #2\rangle^{\Cl}_{#1}}
\newcommand{\Relz}[2]{r}

\newcommand{\model}[1]{\llbracket #1 \rrbracket}
\newcommand{\modelr}[1]{\llbracket #1 \rrbracket_{1}}
\newcommand{\FF}{\mathsf F}
\newcommand{\Rela}[1]{\mathsf{Rel}(#1)}

\newcommand{\Ass}{\B{Ass}(\Lambda)}
\newcommand{\Mod}{\B{Ass}(\Lambda)}

\newcommand{\Assc}[1]{\B{Ass}_{#1}(\Lambda)}
\newcommand{\Modc}[1]{\B{Mod}_{#1}(\Lambda)}

\newcommand{\PER}[1]{\mathsf{PER}_{#1}}
\newcommand{\Fam}{\mathsf{Fam}(\Cl)}
\newcommand{\Set}{\mathsf{Set}}
\newcommand{\Subc}{\mathsf{Sub}(\Cl)}
\newcommand{\Par}[1]{\mathsf{Rel}^{*}(#1)}

\newcommand{\Sub}[1]{\mathsf{Sub}(#1)}

\newcommand{\Assub}{\B{Mod}^{\hookrightarrow}(\Lambda)}


\definecolor{color0}{HTML}{4682B4}

% TODO
\newcommand{\TODO}[1]{{\color{magenta}\bfseries{#1}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: ""
%%% End:


==> packages.tex <==
\usepackage{etex}
 \usepackage{geometry} % see geometry.pdf on how to lay out the page. There's lots.
 \geometry{a4paper} 
 \usepackage{appendix}
% \usepackage{palatino}
%\usepackage{mathpazo}
\usepackage{stackrel}
\usepackage{rotating}
 \usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{amsfonts}
\usepackage{cmll}
\usepackage{amsthm}% or letter or a5paper or ... etc
\usepackage{amsmath}% or letter or a5paper or ... etc
\usepackage{proof}
\usepackage{mathdots}
\usepackage{hyperref}
\usepackage{xcolor}
\usepackage{amssymb}
\usepackage{color}
\usepackage{tikz}
\usepackage{mathrsfs}
\usepackage[all]{xy}
\usepackage{lscape}
\usepackage{stmaryrd}
\usepackage{mathdots}
\usepackage{bbm}
\usepackage{makeidx}
\usepackage{bussproofs}
\usepackage{subcaption}
%\usepackage{mathabx}

\EnableBpAbbreviations

\usetikzlibrary{cd}



%\usepackage{KCP}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: ""
%%% End:

